Surgical Data Science -- from Concepts toward Clinical Translation

Recent developments in data science in general and machine learning in particular have transformed the way experts envision the future of surgery. Surgical Data Science (SDS) is a new research field that aims to improve the quality of interventional healthcare through the capture, organization, analysis and modeling of data. While an increasing number of data-driven approaches and clinical applications have been studied in the fields of radiological and clinical data science, translational success stories are still lacking in surgery. In this publication, we shed light on the underlying reasons and provide a roadmap for future advances in the field. Based on an international workshop involving leading researchers in the field of SDS, we review current practice, key achievements and initiatives as well as available standards and tools for a number of topics relevant to the field, namely (1) infrastructure for data acquisition, storage and access in the presence of regulatory constraints, (2) data annotation and sharing and (3) data analytics. We further complement this technical perspective with (4) a review of currently available SDS products and the translational progress from academia and (5) a roadmap for faster clinical translation and exploitation of the full potential of SDS, based on an international multi-round Delphi process.

==> appendices/initiatives.tex <==
\renewcommand{\appendixtitle}{Surgical Data Science initiatives}
\section*{\appendixtitleFull}
%\section{Surgical Data Science initiatives}
\label{app:initiatives}

\begin{center}
\tablefirsthead{%
  \toprule
  \multicolumn{1}{l}{Project title} &
  \multicolumn{1}{l}{Description} &
  \multicolumn{1}{l}{Funding source} &
  \multicolumn{1}{l}{Period} &
  \multicolumn{1}{l}{Publication} \\
  \midrule }
\tablehead{%
  \midrule
  \multicolumn{5}{l}{\small\sl continued from previous page} \\
  \toprule
  \multicolumn{1}{l}{Project title} &
  \multicolumn{1}{l}{Description} &
  \multicolumn{1}{l}{Funding source} &
  \multicolumn{1}{l}{Period} &
  \multicolumn{1}{l}{Publication} \\
  \midrule }
\tabletail{%
  \midrule
  \multicolumn{5}{r}{\small\sl continued on next page} \\
  \midrule }
\tablelasttail{}
\topcaption{Surgical Data Science initiatives}
\begin{supertabular}{p{3cm} p{4cm} p{4cm} p{1.5cm} p{3cm}}
Surgical Data Science Initiative &
  Surgical data science aims to improve the quality of interventional healthcare and its   value through the capture, organization, analysis and modelling of data. &
  National Center of Tumor Disease (NCT), German Cancer Research Center (DKFZ) &
  since 2015 &
  Maier-Hein, L. 2017 DOI 10.1038/s41551-017-0132-7; Maier-Hein, L. 2018 arXiv:1806.03184; http://www.surgical-data-science.org/ \\
RONNA &
  Upgradeable robotic neuro-navigation system and open for development under the H2020   SurgIOM project &
  ERDF - European   Regional Development Fund {[}2014-2016{]}, Faculty of Mechanical Engineering and   Naval Architecture, Clinical Hospital Dubrava, Croatian Institute for Brain   Research (Croatian Institute of Technology) {[}2011-2013{]} &
  since 2011 &
  Jerbić et al.   2020; Dlaka et al. 2017 \\
Tomorrow’s health Territory - Investment of the future program “Innovative Territory” &
  Innovations for healthcare (real-time access to data, telemedicine, deployment of e-health; Set up of regional digital platform to develop innovative e-health services. &
  Priesm, Better, IHU &
  2020-2024 &
   \\
ARAILIS - Augmented Reality and Artificial Intelligence &
  Research soft-tissue navigation and visualization based on AI-assisted methods &
   &
   &
   \\
supported Laparoscopic Imagery in Surgery &
&
  Sächsische Aufbaubank (SAB) &
  2020-2023 &
   \\
CeTI - Centre for Tactile Internet with Human-in-the-Loop &
  Research   robot-assisted surgery: Prediction of surgical actions for human-machine collaboration and sensor-based surgical training.  &
  German Research Foundation (DFG), EXC 2050/1 &
  2019-2025 &
   \\
CoBot - Colorectal robotic assistant for laparoscopic surgery &
  Research  robot-assisted surgery: Development of context-aware assistance functions for colorectal surgeries &
  Else Kröner   Fresenius Center for Digital Health &
  2019-2021 &
   \\
   SurgOmics &
   Prediction of adverse events in surgery based on the AI-based analysis of process features &
   Federal Ministry of Health (BMG) &
   2020 - 2023 &
   \\
BOOSTER &
  Developing   personalized medicine for strokes in emergency situations to provide faster   and better emergency care to a larger number of stroke victims. &
  INSA INRIA &
  2019-2024 &
   \\
IamRONNA   - Intelligent Autonomous Mobile RONNA &
  Development of   an autonomous omnidirectional mobile platform equipped with a propulsion   system, 3D vision and laser sensors for application to other medical devices   as well as to other tasks within operating rooms and hospital spaces. &
  Adris Foundation &
  2019-2021 &
   \\
CRTA   - Regional Center of Excellence for Robotic Technologies &
  Operating   theatre specialized for neurosurgical applications but also for general   surgery. Validation of concepts of the SurgIOM for neurosurgery and for   sensorization of laparoscopic instruments. &
  ERDF - European   Regional Development Fund &
  2018-2021 &
   \\
Augmented   Reality Surgical System iSurgeon &
  Medical and   technical experts with experience in computer-assisted surgery identified   four research areas with a high potential for sustainably improving surgical   oncology: (1) functional imaging based on biophotonics, (2) multimodal data   visualization through augmented reality, (3) reproducible imaging by means of   robotics, and (4) context-aware visualization based on surgical data science. &
  Federal Ministry   for Economic Affairs and Energy (BMWi) &
  2018-2020 &
  Maier-Hein, L.,   Gockel, I., Speidel, S. et al. Intraoperative Bildgebung und Visualisierung.   Onkologe 26, 31–43 (2020). https://doi.org/10.1007/s00761-019-00695-4 \\
NERO   - Neurosurgical Robot &
  Development of   head phantoms and base frames for stereotactic neurosurgery. &
  ERDF - European   Regional Development Fund &
  2017-2021 &
   \\
OP 4.1 Smart Services II &
  Concept for the   design of a platform to bring apps (software innovation) into the operating   room. &
  Federal Ministry   for Economic Affairs and Energy (BMWi) &
  08/2017-02/2020 &
  OP 4.1: A   User-Centered Platform for the Operation Room of the Future K. März, L.   Mündermann, M. Nolden, T. Simpfendörfer, C. Gasch, T. Ross, S. Onogur, J.   Metzger, C. Feldmann, J. Fallert, M. Hohenfellner, L. Maier-Hein {[}IPCAI 2019{]} \\
FastPath   - Innovative pathways for minimally invasive surgery patients &
  Innovative   patient care pathways adapted to image guided minimally invasive surgery and   methods measure relevant patient and health economics outcomes. &
  IHU, Medtronic &
  01/2016-01/2021 &
   \\
DeepSurg   - ANR JCJC - National Project &
  AI/DL methods   for the analysis of clinical activities in hybrid procedures using multiple   RGBD ceiling-mounted cameras &
  UNISTRA, IHU &
  2016-2021 &
   \\
CONDOR - Connected Optimized Network \& Data in Operating Rooms. Video standards   \& infra-structure in Operating Room &
  Video standard   and infrastructure for the recording and live streaming of surgical data and   metadata. Computer vision tools for the analysis of surgery &
  BPI France, IHU,   UNISTRA &
  10/2016-09/2020 &
   \\
InnOPlan,   Smart Data Technologies &
  Concepts for   connecting devices and IT-Systems and resulted in a smart data platform. &
  BMWi &
  01/2015-03/2018 &
   \\
ACRON   - A new concept of Applied Cognitive RObotics in clinical Neuroscience &
  Novel algorithms   (Šuligoj et al. 2017; 2018) for precise patient localization in neurosurgery   from the ACRON project will be used in the SurgIOM project for maximally   automating certain steps of the neurosurgical procedure. &
  Croatian Science   Foundation (HRZZ) &
  2014-2018 &
   \\
Endoscopy meets computer science: Precise navigation for minimally-invasive surgery &
   &
  Klaus Tschira Stiftung &
  2014-2016 &
   \\
DFG Collaborative Research Project (SFB) 125: Cognition-guided surgery:    “Knowledge-based navigated liver surgery” &
   &
  Deutsche Forschungsgemeinschaft (DFG) &
  07/2012-06/2017 &
   \\
DFG   Research Training Group 1126: Intelligent Surgery: “Planning and navigation   in ablation therapy” (PI) &
   &
  DFG &
  06/2012-03/2014 &
   \\
DFG   Research Training Group 1126: Intelligent Surgery: “Navigated liver   resection” (PI) &
   &
  DFG &
  06/2012-03/2014 &
   \\
OR.NET   - Secure dynamic networking in the operating room and clinic &
  Cross-vendor   concepts and standards (IEEE 11073 SDC) for the dynamic and secure networking   of medical devices and IT systems in the OR and in clinics. &
  BMBF &
  09/2012-04/2016 &
   \\
X-RAIS &
  AI tool for the   analysis of medical images based on neural networks and Radiomics techniques. &
  SRY &
   &
   \\
Smart   Image &
  The advent of   laparoscopic cholecystectomy almost 30 years ago would change forever the way   surgeons visualize and interact with target anatomy Patients continue to   benefit from different yet related image guided therapies that also allow   access to pathology by minimally invasive means.  As we continue to   depend upon images to guide and inform patient interventions it is   instructive to review the advances made in surgical visualization over its   recent history and look forward to issues that will need to be addressed   toward optimization of interventional visualization.  These issues will   be reviewed from the perspective of a clinician,  not a computer scientist   nor a physicist, with attention also paid to the often neglected topics of   ergonomics and human factors considerations in surgical visualization. &
   &
   &
   \\
OR Black Box: using data to improve surgical safety &
  OR Black Box aims to improve patient safety and outcomes by characterizing intraoperative errors, events, and distractions which allows better surgical coaching and improvements. This product records synchronized data of multiple sensor feeds in the OR such as the video of the surgical scene, audio of the conversations among the surgical team, patient vital signs, feedback from electronic surgical instruments, and analyses the recorded data to provide comprehensive, objective, and clinically relevant insights into the perioperative environment. &
   &
  2017 &
  M. G. Goldenberg, J. Jung, and T. P. Grantcharov, “Using Data to Enhance Performance and Improve Quality and Safety in Surgery,” JAMA Surg., vol. 152, no. 10, pp. 972–973, 01 2017, doi: 10.1001/jamasurg.2017.2888.\newline
  J. J. Jung, P. Jüni, G.   Lebovic, and T. Grantcharov, “First-year Analysis of the Operating Room Black   Box Study,” Ann. Surg., vol. 271, no. 1, pp. 122–127, 2020, doi:   10.1097/SLA.0000000000002863.\\
AI4OR,   A Network Initiative for Context-Aware Operating Theaters &
  Create   innovative solutions to context-awareness in operating theaters, with a   particular focus on surgical process modeling, analysis and recognition of   surgical processes, and cognitive surgical robotics, primarily using AI algorithms &
   &
  since 2018 &
   \\
Multidisciplinary Computational Anatomy (MCA) &
  Multidisciplinary Computational Anatomy (MCA) supported by the Japan MEXT grant has been   established to integrate the medical images with information along four axes such as time, space, function and pathology. MCA model is a prediction model of those information with medical images. MCA-based medicine with AI is one of the solutions to solve the difficulties of current medical problems. &
   &
  since 2017 &
   \\
SAGES AI Taskforce &
   &
   &
   &
   \\
CARSS Initiative &
   &
   &
   &
   \\
SAGES Video Annotation Consensus Conference &
   &
   &
   &
   \\
\bottomrule
\end{supertabular}
\label{tab:initiatives}
\end{center}


==> appendices/questionnaire.tex <==
\renewcommand{\appendixtitle}{Questionnaire}
\section*{\appendixtitleFull}
%\section{Questionnaire}
\label{app:questionnaire}

\begin{center}
%\sffamily\small
\tablefirsthead{%
  \toprule
  \multicolumn{1}{l}{ID} &
  \multicolumn{1}{l}{Question} \\
  \midrule }
\tablehead{%
  \midrule
  \multicolumn{2}{l}{\small\sl continued from previous page} \\
  \toprule
  \multicolumn{1}{l}{ID} &
  \multicolumn{1}{l}{Question} \\
  \midrule }
\tabletail{%
  \midrule
  \multicolumn{2}{r}{\sffamily\small\sl continued on next page} \\
  \midrule }
\tablelasttail{}
\topcaption{Questions along with the workshop registration form.}
\sffamily\small
\begin{supertabular}{p{0.6cm} p{14cm}}
\multicolumn{2}{l}{General information} \\
\midrule
Q01 &
What is your background?\newline
Options (multiple selections allowed):
\begin{itemize}
\item Academic: Clinical
\item Academic: Engineering
\item Clinical
\item Industrial
\item Other
\end{itemize}
\\
Q02 &
What is your role?\newline
Options (single selection):
\begin{itemize}
\item Board member/member of organizing committee
\item Professor/Academic group leader
\item Industry
\item PhD Student
\item Undergraduate
\item Postdoc
\item Other
\end{itemize}
\\
Q03 &
Do you want to be acknowledged in a publication of the workshop results?\newline
Options: Yes or No
\\
Q04 &
What is your main incentive for registration to the workshop?\newline
Options (single selection and/or free text):
\begin{itemize}
\item Learning about SDS
\item Meeting SDS experts/networking
\item Advancing the field
\item Being part of the upcoming paper
\item Other (please specify)
\end{itemize}
\\ \midrule
\multicolumn{2}{l}{Successes related to Surgical Data Science}
\\ \midrule
Q05 &
Please name a prominent surgical data science \enquote{success story} (e.g. a clinical application that has been shown to benefit from surgical data science or new insights that were generated based on surgical data science techniques). Describe what you mean by success in this case.
\\
Q06 &
Which research paper in the field of surgical data science has impressed you the most so far?
\\ \midrule
\multicolumn{2}{l}{Challenges related to Surgical Data Science}
\\ \midrule
Q07 &
What are the most critical challenges related to exploiting the potential of surgical data science?
\\
Q08 &
What is lacking in the existing public data sets?
\\
Q09 &
What do you consider as the most urgent issue/problem that needs to be discussed in the workshop (e.g. standards)?
\\ \midrule
\multicolumn{2}{l}{Future of Surgical Data Science}
\\ \midrule
Q10 &
Please list at least one surgical data science (clinical) application that can be regarded as a (relatively) low hanging fruit (i.e. could be addressed in a relatively short period of time).
\\
Q11 &
What should be the next SDS challenge (open competition)?
\\ \midrule
\multicolumn{2}{l}{Personal experience with Surgical Data Science}
\\ \midrule
Q12 &
What public data set have you found the most useful for your research in SDS so far?
\\
Q13 &
What was your biggest failure in SDS, even though it looked promising at the beginning, to avoid others making the same mistake?
\\
Q14 &
What is your advice for avoiding these problems?
\\ \midrule
\multicolumn{2}{l}{Joint Surgical Data Science Project}
\\ \midrule
Q15 &
Would you be interested to work on a joint surgical data science project with other workshop attendees?
\\
Q16 &
Do you (potentially) have data to contribute to such a project?
\\
Q17 &
If yes, what kind of data?
\\ \midrule
\multicolumn{2}{l}{Where do we stand?}
\\ \midrule
Q18 &
What do you regard as the most important developments in the field since the last workshop in June 2016?
\\
Q19 &
Surgical Data Science failures: Are you aware of projects that have failed (optionally and preferably: name them)?
\\
Q20 &
What was the (main) reason for failure?
\\
\bottomrule
\end{supertabular}
\label{tab:questionnaire}
\end{center}


==> appendices/questionnaireResults.tex <==
\renewcommand{\appendixtitle}{Results of questionnaire}
\section*{\appendixtitleFull}
%\section{Results of questionnaire}
\label{app:questionnaireResults}

\subsection{General information}

\noindent \newline \textit{\textbf{Q01:} What is your background?}

\begin{figure}[pos=h]
  \begin{subfigure}[c]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim=4cm 1cm 4cm 1cm, clip]{figures/q01_background_plot.pdf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.59\textwidth}
    \includegraphics[height=5cm, trim=4.5cm 2cm 0cm 2cm, clip]{figures/q01_background_legend.pdf}
  \end{subfigure}
\end{figure}

\noindent \textit{\textbf{Q02:} What is your role?}

\begin{figure}[pos=h]
  \begin{subfigure}[c]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim=4cm 1cm 4cm 1cm, clip]{figures/q02_roles_plot.pdf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.59\textwidth}
    \includegraphics[height=5cm, trim=4cm 2cm 0cm 2cm, clip]{figures/q02_roles_legend.pdf}
  \end{subfigure}
\end{figure}

\noindent \textit{\textbf{Q03:} Do you want to be acknowledged in a publication of the workshop results?}

\begin{figure}[pos=h]
  \begin{subfigure}[c]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim=4cm 1cm 4cm 1cm, clip]{figures/q03_acknowledgment_in_publication.pdf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.59\textwidth}
    \includegraphics[height=5cm]{figures/blank.pdf}
  \end{subfigure}
\end{figure}

\newpage
\noindent \textit{\textbf{Q04:} What is your main incentive for registration to the workshop?}

\begin{figure}[pos=h]
  \begin{subfigure}[c]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim=4cm 1cm 4cm 1cm, clip]{figures/q04_incentive_for_registration_plot.pdf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.59\textwidth}
    \includegraphics[height=5cm, trim=5.5cm 2cm 0cm 2cm, clip]{figures/q04_incentive_for_registration_legend.pdf}
  \end{subfigure}
\end{figure}

\subsection{Successes related to Surgical Data Science}

\noindent \newline \textit{\textbf{Q05:} Please name a prominent surgical data science \enquote{success story} (e.g. a clinical application that has been shown to benefit from surgical data science or new insights that were generated based on surgical data science techniques). Describe what you mean by success in this case.}

\noindent \newline 87\% of participants responded to this question. 81 partial replies were extracted from the free text and categorized. Of these, 68\% named projects, systems, and (fields of) applications in different levels of detail. The most prominent project is the OR Black Box led by \citeappendix{appendix:goldenberg_using_2017} (7 mentions). Surgical workflow analysis is the most promising field of application (4 mentions), followed by the work of the \citeappendix{appendix:camma_camma_nodate} group (3 mentions). 9\% mentioned that they were not aware of any success story. Participants were also struggling with the definition of a \enquote{success story} in the field of surgical data science and came up with definitions of what success is in their understanding (17\%).

\begin{figure}[pos=h]
  \begin{subfigure}[c]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim=4cm 1cm 4cm 1cm, clip]{figures/q05_success_stories_plot.pdf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.59\textwidth}
    \includegraphics[height=5cm, trim=5.5cm 2cm 0cm 2cm, clip]{figures/q05_success_stories_legend.pdf}
  \end{subfigure}
\end{figure}

\noindent \textit{\textbf{Q06:} Which research paper in the field of surgical data science has impressed you the most so far?}

\noindent \newline 80\% of the participants responded to this question. 62 partial replies were extracted from the free text and categorized. 81\% of the replies contained references to identifiable publications. The most frequently named publication was \citeappendix{appendix:maier-hein_surgical_2017} (30\%), which originated from the first workshop on surgical data science. 80\% of these nominations were from participants that did not author this paper. With two nominations \citeappendix{appendix:shademan_supervised_2016} was the second most named publication. All other publications were nominated once.

\newpage
\subsection{Challenges related to Surgical Data Science}

\noindent \newline \textit{\textbf{Q07:} What are the most critical challenges related to exploiting the potential of surgical data science?}

\noindent \newline 90\% of participants responded to this question. 142 partial replies were extracted from the free text and categorized.

\begin{figure}[pos=h]
  \begin{subfigure}[c]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim=4cm 1cm 4cm 1cm, clip]{figures/q07_most_critical_challenges_plot.pdf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.59\textwidth}
    \includegraphics[height=8cm, trim=4cm 0cm 0cm 0cm, clip]{figures/q07_most_critical_challenges_legend.pdf}
  \end{subfigure}
\end{figure}

\noindent \textit{\textbf{Q08:} What is lacking in the existing public data sets?}

\noindent \newline 81\% of participants responded to this question. 82 partial replies were extracted from the free text and categorized.

\begin{figure}[pos=h]
  \begin{subfigure}[c]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim=4cm 1cm 4cm 1cm, clip]{figures/q08_lack_in_public_data sets_plot.pdf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.59\textwidth}
    \includegraphics[height=5cm, trim=5.5cm 2cm 0cm 2cm, clip]{figures/q08_lack_in_public_data sets_legend.pdf}
  \end{subfigure}
\end{figure}

\newpage
\noindent \textit{\textbf{Q09:} What do you consider as the most urgent issue/problem that needs to be discussed in the workshop (e.g. standards)?}

\noindent \newline 84\% of participants responded to this question. 96 partial replies were extracted from the free text and categorized.

\begin{figure}[pos=h]
  \begin{subfigure}[c]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim=4cm 1cm 4cm 1cm, clip]{figures/q09_most_urgent_issues_plot.pdf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.59\textwidth}
    \includegraphics[height=5cm, trim=4.5cm 2cm 0cm 2cm, clip]{figures/q09_most_urgent_issues_legend.pdf}
  \end{subfigure}
\end{figure}

\noindent \textit{\textbf{Q10:} Please list at least one surgical data science (clinical) application that can be regarded as a (relatively) low hanging fruit (i.e. could be addressed in a relatively short period of time).}

\noindent \newline 79\% of participants responded to this question. 70 partial replies were extracted from the free text and categorized. Of these, 7\% expressed doubts that low hanging fruit exist. 92\% of the replies contained fields and applications of low hanging fruit, including instrument segmentation, skill assessment and training, tracking, prediction of outcome and duration as well as sharing data and tools. These sub-categories were nominated more than twice. 1\% of the replies contained a definition of high hanging fruit.

%\vspace{\baselineskip}

\noindent \newline \textit{\textbf{Q11:} What should be the next SDS challenge (open competition)?}

\noindent \newline 71\% of participants responded to this question. 67 partial replies were extracted from the free text and categorized. Of these, 40\% of replies contain nominations of challenges that cannot be assigned to any of the categories.

\begin{figure}[pos=h]
  \begin{subfigure}[c]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim=4cm 1cm 4cm 1cm, clip]{figures/q11_next_open_competitions_plot.pdf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.59\textwidth}
    \includegraphics[height=5cm, trim=6.5cm 2cm 0cm 2cm, clip]{figures/q11_next_open_competitions_legend.pdf}
  \end{subfigure}
\end{figure}

\newpage
\subsection{Personal experience with Surgical Data Science}

\noindent \newline \textit{\textbf{Q12:} What public data set have you found the most useful for your research in SDS so far?}

\noindent \newline 79\% of participants responded to this question. 82 partial replies were extracted from the free text and categorized. Of these, 71\% contained references to identifiable data sets (either general collections or subsets). 29\% contained other responses, e.g. including non-identifiable data sets, persons stating that they are not able to name one, because they are new to the field or they were using private data sets so far. Among the identifiable data sets, \citeappendix{appendix:endovis_endovis_nodate} was most frequently named (28\%). With 21\% of nominations Cholec80 \citepappendix{appendix:twinanda_endonet_2017} is the second most named data set, followed by JIGSAWS \citepappendix{appendix:gao_jhu-isi_2014} (17\%). Four data sets were named twice. 21\% of data sets were named once.

\noindent \newline \textit{\textbf{Q13:} What was your biggest failure in SDS, even though it looked promising at the beginning, to avoid others making the same mistake?}

\noindent \newline 68\% of participants were able to name a failure in SDS. 52 partial replies were extracted from the free text and categorized. Of these, 10\% contained references to non-identifiable projects 32\% of participants did not provide an answer for various reasons (e.g. confidentiality, novice in field).

\begin{figure}[pos=h]
  \begin{subfigure}[c]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim=4cm 1cm 4cm 1cm, clip]{figures/q13_personal_failures_plot.pdf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.59\textwidth}
    \includegraphics[height=5cm, trim=4.5cm 2cm 0cm 2cm, clip]{figures/q13_personal_failures_legend.pdf}
  \end{subfigure}
\end{figure}

\noindent \newline \textit{\textbf{Q14:} What is your advice for avoiding these problems?}

\noindent \newline 64 partial replies were extracted from the free text and categorized. 25\% of these replies recommend to collaborate (early) with different stakeholders (e.g. clinicians, statisticians, technology experts) to succeed in SDS projects. Having access to more data in general (17\%) and investing in a robust infrastructure for data acquisition (6\%) as well as high-quality annotations (5\%) specifically is also advised. Defining smaller project goals (9\%) can help to identify pitfalls. Topics related to education and dissemination (e.g. understanding well-posedness of a problem) (8\%) as well as proper validation (5\%) are also covered by the participants’ advice.

\begin{figure}[pos=h]
  \begin{subfigure}[c]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim=4cm 1cm 4cm 1cm, clip]{figures/q14_personal_advice_plot.pdf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.59\textwidth}
    \includegraphics[height=5cm, trim=5.2cm 2cm 0cm 2cm, clip]{figures/q14_personal_advice_legend.pdf}
  \end{subfigure}
\end{figure}

\subsection{Joint Surgical Data Science Project}

\noindent \newline \textit{\textbf{Q15:} Would you be interested to work on a joint surgical data science project with other workshop attendees?}

\begin{figure}[pos=h]
  \begin{subfigure}[c]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim=4cm 1cm 4cm 1cm, clip]{figures/q15_joint_project.pdf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.59\textwidth}
    \includegraphics[height=5cm]{figures/blank.pdf}
  \end{subfigure}
\end{figure}

\noindent \textit{\textbf{Q16:} Do you (potentially) have data to contribute to such a project?}

\begin{figure}[pos=h]
  \begin{subfigure}[c]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim=4cm 1cm 4cm 1cm, clip]{figures/q16_data_contribution.pdf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.59\textwidth}
    \includegraphics[height=5cm]{figures/blank.pdf}
  \end{subfigure}
\end{figure}

\noindent \textit{\textbf{Q17:} If yes, what kind of data?}

\noindent \newline The kind of data was specified in different levels of detail (e.g. from single words describing the format to more detailed descriptions of the anatomical structures, devices, modalities and parameters used for data acquisition). This is due to the open formulation of the question. The level of detail was not specified. 45\% of participants opted for “Yes”. 11\% of these did not specify the kind of data. 42\% of participants opted for “No”. Of these, 6\% specified the kind of data and 3\% specified a reason.

\newpage
\subsection{Where do we stand?}

\noindent \newline \textit{\textbf{Q18:} What do you regard as the most important developments in the field since the last workshop in June 2016?}

\noindent \newline 38\% of participants responded to this question. 36 partial replies were extracted from the free text and categorized.

\begin{figure}[pos=h]
  \begin{subfigure}[c]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim=4cm 1cm 4cm 1cm, clip]{figures/q18_important_developments_plot.pdf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.59\textwidth}
    \includegraphics[height=5cm, trim=4.5cm 2cm 0cm 2cm, clip]{figures/q18_important_developments_legend.pdf}
  \end{subfigure}
\end{figure}

\noindent \textit{\textbf{Q19:} Surgical Data Science failures: Are you aware of projects that have failed (optionally and preferably: name them)?}

\noindent \newline 27\% of participants were aware of at least one project that failed, yielded to 28 failing projects in total. IBM Watson was the only project mentioned multiple times (which is not even a SDS project). 73\% of participants did not name or were not aware of any failing project. Of these, 5\% still named reasons for failures.

\vspace{\baselineskip}

\noindent \textit{\textbf{Q20:} What was the (main) reason for failure?}

\begin{figure}[pos=h]
  \begin{subfigure}[c]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim=4cm 1cm 4cm 1cm, clip]{figures/q20_reasons_for_failures_plot.pdf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.59\textwidth}
    \includegraphics[height=5cm, trim=4.5cm 2cm 0cm 2cm, clip]{figures/q20_reasons_for_failures_legend.pdf}
  \end{subfigure}
\end{figure}


==> tables/contextStatement.tex <==
\begin{table}

\caption{\textcolor{red}{UNDER REVISION: Context Statement.}}
\begin{tcolorbox}[title= Context Statement, colback=white, halign=left, subtitle style={boxrule=0.4pt,colback=gray}]
    %\hspace{-0.5cm}
    %\textcolor{red}{
    Unless otherwise specified, in all of the following text, a) surgical data science (SDS) represents the general context of the suggested phrases and b) “data” may pertain to any part of the patient care process (from initial presentation to long-term outcomes), may concern the patient, caregivers and/or technology used to deliver care and must be acquired, stored, and shared in accordance with both local and international regulatory constraints. Finally, c) the term SDS stakeholders refers to clinical, research, public, regulatory and industrial stakeholders.
    %}
\end{tcolorbox}
\label{tab:contextStatement}
\end{table}
